Modeling optical and UV polarization of AGNs

Optical observations cannot resolve the structure of active galactic nuclei (AGN), and a unified model for AGN was inferred mostly from indirect methods. Optical reverberation mapping allowed us to constrain the spatial dimension of the broad emission line region and thereby to measure the mass of supermassive black holes. Recently, reverberation was also applied to the polarized signal emerging from different AGN components. In principle, this should allow us to measure the spatial dimensions of the sub-parsec reprocessing media. We modeled scattering-induced polarization and tested different geometries for the circumnuclear dust component. Our tests included the effects of clumpiness and different dust prescriptions. To further extend the model, we also explored the effects of additional ionized winds stretched along the polar direction, and of an equatorial scattering ring that is responsible for the polarization angle observed in pole-on AGN. The simulations were run using a time-dependent version of the {\sc stokes} code. Our modeling confirms the previously found polarization characteristics as a function of the observer`s viewing angle. When the dust adopts a flared-disk geometry, the lags reveal a clear difference between type 1 and type 2 AGN. This distinction is less clear for a torus geometry where the time lag is more sensitive to the geometry and optical depth of the inner surface layers of the funnel. The presence of a scattering equatorial ring and ionized outflows increased the recorded polarization time lags, and the polar outflows smooths out dependence on viewing angle. Together with other AGN observables, the polarization time lag places new, independent constraints on the inner geometry of AGN. If we conduct time-dependent spectropolarimetric observing campaigns of AGN, this method has a high potential for a census of supermassive black holes.

==> bibliography_manual.tex <==
\begin{thebibliography}{}


  \bibitem[Afanasiev et al.(2015)]{Afanasiev2015} Afanasiev, V.~L., Shapovalova, A.~I., Popovi{\'c}, L.~{\v C}., \& Borisov, N.~V.\ 2015, \mnras, 448, 2879 

  \bibitem[Afanasiev et al.(2014)]{Afanasiev2014} Afanasiev, V.~L., Popovi{\'c}, L.~{\v C}., Shapovalova, A.~I., Borisov, N.~V., \& Ili{\'c}, D.\ 2014, \mnras, 440, 519 

  \bibitem[Antonucci (1984)]{Antonucci1984} Antonucci, R. 1984, ApJ, 278, 499
  
  \bibitem[Antonucci (1993)]{Antonucci1993} Antonucci, R. 1993, \araa, 31, 473
  
  \bibitem[Antonucci (1994)]{Antonucci1994} Antonucci, R. 1994, A\&A, 31, 473
 
  \bibitem[Antonucci and Miller (1985)]{Antonucci1985} Antonucci, R. and   Miller, J.S., 1985, ApJ, 297, 621A 
  
  \bibitem[Batcheldor et al. (2011)]{Batcheldoretal2011} Batcheldor, D., Robinson, A.,Axon, D. J., Young, S., Quinn, S., Smith, J. E., Hough, J. and  Alexander, D. M. 2011, ApJ, 738, 90B  
     
  \bibitem[Gaskell (2009)]{Gaskell2009} Gaskell, C. M. 2009, NewAR 53, 140

  \bibitem[Gaskell(1982)]{Gaskell1982} Gaskell, C.~M.\ 1982, ApJ, 263, 79 

  \bibitem[Gaskell \& Goosmann(2013)]{Gaskell2013} Gaskell, C.~M., \& Goosmann, R.~W.\ 2013, ApJ, 769, 30 

  \bibitem[Gaskell and Goosmann (2012)]{GG2012} Gaskell, C. M. and Goosmann, R. W. 2012, ApJ, 769, 30
    
  \bibitem[Gaskell et al. (2012)]{Gaskelletal2012} Gaskell, C. M. and Goosmann, R. W. and Merkulova, N. I. and Shakhovskoy, N. M. and Shoji,
  M. 2012, ApJ, 749, 148
    
  \bibitem[Gaskell et al.(2008)]{Gaskell2008} Gaskell, C.~M., Goosmann, R.~W., \& Klimek, E.~S.\ 2008, MmSAI, 79, 1090 

  \bibitem[Gaskell et al.(2004)]{Gaskell2004} Gaskell, C. M., Goosmann, R. W., Antonucci, R. R. J., \& Whysong, D., 2004, ApJ, 616, 147
  
  \bibitem[Goosmann and Gaskell (2007)]{GG2007} Goosmann, R. W.and Gaskell, C. M. 2007, A\&A, 465, 129 
  
  \bibitem[H{\"o}nig and Kishimoto (2010)]{HonigHashimoto2010} H{\"o}nig, S. and Kishimoto, M. 2010, A\&A, 523A, 27H
  
  \bibitem[Kartje (1995)]{Kartje1995} Kartje, John F. 1995, ApJ, 452, 565.
  
  \bibitem[King and Pounds (2003)] {KingPounds2003} King, A.~R. and Pounds, K.~A. 2003, MNRAS, 345, 657
  
  \bibitem[Kishimoto et al (2013)] {Kishimotoetal2013} Kishimoto, M., H{\"o}nig, S.F., Antonucci, R., Millan-Gabet, R., Barvainis, R., Millour, F., Kotani, T., Tristram, K. R.W. and  Weigelt, G. 2013, ApJ, 775L, 36K
   
  \bibitem[Lynden-Bell (1969)]{lyndenbell1969} Lynden-Bell, D. 1969, Nature 223, 690
  
  \bibitem[Marin et al. (2012)]{Marinetal2012} Marin, M., Goosmann, R. W., Gaskell, C. M., Porquet, D. and Dovciak, M. 2012, A\&A, 548, 121
  
  \bibitem[Marin \& Goosmann(2014)]{MarinGoosmann2014} Marin, F., \& Goosmann, R.~W.\ 2014, SF2A-2014: Proceedings of the Annual meeting of the French Society of Astronomy and Astrophysics, 103 
  
  \bibitem[Marin (2014)]{Marin2014} Marin, F. 2014, MNRAS, 441, 551M
  
  \bibitem[Marin, Goosmann and Gaskell (2015)]{MGG2015} Marin, F., Goosmann, R. W. and Gaskell, C. M. 2015, A\&A, 577, 66 

  \bibitem[Marin (2016)]{Marin2016} Marin, F. 2016, MNRAS 460, 3679M
  
  \bibitem[Mathis, Rumpl \& Nordsieck(1977)]{Mathis1977} Mathis, J. S., Rumpl, W., \& Nordsieck, K. H., 1977, \apj, 217, 425
  
  \bibitem[Nenkova et al.(2008)]{Nenkova2008} Nenkova, M. and Sirocky, M.~M. and Nikutta, R. and Ivezi{\'c}, \v Z. and  Elitzur, M. 2008, ApJ, 685, 160N
  
  \bibitem[Pounds and Page (2006)]{Pounds2006} Pounds K. A. and Page, K. L. 2006, MNRAS, 372, 1275
  
  \bibitem[Pringle, Rees and Pacholczyk (1973)]{prp1973} Pringle, J. E. and Rees, M. J. and Pacholczyk, A. G., 1973, A\&A, 29, 179
  
  \bibitem[Raban et al. (2009)]{Raban2009} Raban, D. and Jaffe, W. and R{\"o}ttgering, H. and Meisenheimer, K. and Tristram, K. R. W. 2009, MNRAS, 394, 1325
 
  \bibitem[Ruiz et al. (2003)]{Ruiz2003} Ruiz, M. and Young, S. and Packham, C. and Alexander, D. M. and Houghg, J. H. 2003, MNRAS, 340, 733R  
  
  \bibitem[Salpeter (1964)]{salpeter1964} Salpeter, E. E. 1964, ApJ, 140, 796 
   
  \bibitem[Shakura and Sunyaev (1973)]{ss1973} Shakura, N. I. and  Sunyaev, R. A. 1973, A\&A, 24, 337

  \bibitem[Shields (1978)]{shields1978} Shields, G. A., 1978, Nature, 272, 706 
     
  \bibitem[Siebenmorgen et al. (2015)]{Siebenmorgen2015} Siebenmorgen, R. and Heymann, F. and Efstathiou, A. 2015,  A\&A,583, A120
  
  \bibitem[Smith et al. (2002)]{Smithetal2002} Smith, J. E., Young, S., Robinson, A., Corbett, E. A., Giannuzzo, M. E., Axon, D. J. and Hough, J.H. 2002, MNRAS, 335, 773S 
   
  \bibitem[Smith et al. (2004)]{Smithetal2004} Smith, J. E. et al., 2004, MNRAS, 350, 1405 
  
  \bibitem[Tombesi et al.(2012)]{Tombesi2012} Tombesi, F. and Cappi, M. and Reeves, J. N. and Braito, V. 2012, MNRAS, 422, 1
  
  \bibitem[Tristram et al. (2007)]{Tristram2007} Tristram, K. R. W. and Meisenheimer, K. and Jaffe, W. and 	Schartmann, M. and Rix, H.-W. and Leinert, C. and Morel, S. and Wittkowski, M. and R{\"o}ttgering, H. and Perrin, G. and Lopez, B. and Raban, D. and Cotton, W. D. and Graser, U. and Paresce, F. and Henning, T. 2007. A\&A, 474, 837
  
  \bibitem[Tristram et al. (2014)]{Tristram2014} Tristram, K. R. W. and Burtscher, L. and Jaffe, W. and Meisenheimer, K. and H{\"o}nig, S. F. and Kishimoto, M. and Schartmann, M. and Weigelt, G. 2014, A\&A, 563,82
	
  %%%%%%%%%%%%%%%%%%%%%%%%%

\end{thebibliography}
